Precision Rosenbluth Measurement of the Proton Elastic Electromagnetic Form Factors and Their Ratio at Q^2 = 2.64, 3.20, and 4.10 GeV^2

Due to the inconsistency in the results of the GEp/Gmp ratio of the proton, as extracted from the Rosenbluth and recoil polarization techniques, high precision measurements of the e-p elastic scattering cross sections were made at Q^2 = 2.64, 3.20, and 4.10 GeV^2. Protons were detected, in contrast to previous measurements where the scattered electrons were detected, which dramatically decreased epsilon-dependent systematic uncertainties and corrections. A single spectrometer measured the scattered protons of interest while simultaneous measurements at Q^2 = 0.5 GeV^2 were carried out using another spectrometer which served as a luminosity monitor in order to remove any uncertainties due to beam charge and target density fluctuations. The absolute uncertainty in the measured cross sections is \approx 3% for both spectrometers and with relative uncertainties, random and slope, below 1% for the higher Q^2 protons, and below 1% random and 6% slope for the monitor spectrometer. The extracted electric and magnetic form factors were determined to 4%-7% for GEp and 1.5% for GMp. The ratio GEp/Gmp was determined to 4%-7% and showed mu_p GEp/GMp \approx 1.0. The results of this work are in agreement with the previous Rosenbluth data and inconsistent with high-Q^2 recoil polarization results, implying a systematic difference between the two techniques.

==> proton_absorption_bck.tex <==
\newpage
\section{Proton Absorption} \label{proton_absorp}

Once the protons are struck, they have to travel through material
in the target, spectrometer, and the detector stack before they can 
cause a trigger in the scintillators. While traveling, some protons undergo nuclear 
interaction in these materials and hence get absorbed or scattered. 
Such loss due to the nuclear interaction is called nuclear absorption. 
In order to determine the proton absorption for each arm, we have to account for all the 
target materials the protons have to pass through on their way to the scintillators. 
Also the thickness \cite{alcorn04,schultethesis,lingyanzhuthesis,jones_priv,arrington_priv} and 
density of each absorber \cite{hagiwara02,eidelman04,schultethesis,lingyanzhuthesis}, and the mean 
free path between nuclear collision $\bar{\lambda}$ (effective absorption length) are needed 
in order to calculate the absorption. 

To determine $\bar{\lambda}$, the mean free path between nuclear collision (total interaction
length), $\lambda_{T}$, and the mean free path between inelastic interactions 
(inelastic interaction length), $\lambda_{I}$, must be known \cite{hagiwara02,eidelman04} . 
In the analysis of the E01-001 experiment, $\bar{\lambda}$ was determined using two different definitions. 
The first definition, $\bar{\lambda}$ is estimated as $2\lambda_{T}\lambda_{I}/(\lambda_{T}+\lambda_{I})$ 
assuming that half of the elastic and inelastic scattering contribute to the absorption. 
The second definition, $\bar{\lambda}$ is estimated as the average of two lengths or 
($\lambda_{T}+\lambda_{I}$)/2 since we cannot determine exactly the full contribution from the elastic 
scattering to the absorption. I will refer to $\bar{\lambda}$ estimated by the first(second) definition 
as $\lambda_{act}$($\lambda_{avg}$) where $act$ and $avg$ stand for actual and average. 

The ratio of $X/\bar{\lambda}$ is calculated for each absorber first using $\lambda_{act}$
and then $\lambda_{avg}$. Here $X$ is the product of the absorber's density and thickness. The ratios 
are then added, i.e, $\sum_{i=1}^n (X_{i}/\bar{\lambda_{i}})$ where $i$ runs over all absorbers $n$.  
The proton absorption is given by:
%
\begin{equation}
\mbox{proton absorption} = 1.0 - e^{-\sum_{i=1}^n (X_{i}/\bar{\lambda_{i}})}~, 
\end{equation}
%
where $e^{-\sum_{i=1}^n (X_{i}/\bar{\lambda_{i}})}$ defines the proton transmission. 
The final proton absorption used is the average value of the calculated proton absorption from 
the two definitions or 5.19\% for the right arm and 4.91\% for the left arm giving a proton 
absorption correction of $C_{Absorption}$ = 0.948 and 0.951 for the right arm and left arm, 
respectively. Tables \ref{r_proton_absorp} and \ref{l_proton_absorp} list the absorbers used and their 
properties for both arms. Uncertainty in the final proton absorption used rise due to our lack of precise 
knowledge of the actual thickness of each absorber used and the use of different cross sections in determining 
the mean free path lengths discussed above. Therefore, a scale offset of 1\% is assigned. 
Due to the fact that the scattered proton will have to travel different path length inside the LH$_2$ 
target at each kinematics, calculations of the proton absorption inside the LH$_2$ target at different 
scattering angles for both arms show an $\varepsilon$ dependence uncertainty of 0.03\% and 0.10\% for the
left and right arm, respectively. Random uncertainty of 0.0\% is assigned. 
%%%%
\begin{table}[!htbp]
\begin{center}
\begin{tabular}{||c|c|c|c|c||}
\hline \hline
Target&Density&Thickness&X&$\lambda_T$\\
      &(gm/cm$^3$)&(cm)&(gm/cm$^2$)&(gm/cm$^2$)\\
\hline \hline
LH$_2$ Target&0.708E-01&1.69934&0.1203&43.30\\
Al Target&2.70&0.164484E-01&0.444E-01&70.60\\
Al Chamber&2.70&0.33E-01&0.891E-01&70.60\\
Kapton&1.42&0.254E-01&0.361E-01&60.30\\
Titanium&4.54&0.10E-01&0.454E-01&79.90\\
Air (Spectrometer exist to VDC1)&0.121E-02&80.00&0.968E-01&62.00\\
Mylar (Wire Chamber)&1.39&0.12E-01&0.167E-01&62.50\\
Wire VDC (effective)&19.30&0.40E-04&0.772E-03&110.30\\
Ar/Ethan&0.107E-02&20.00&0.214E-01&68.572\\
S$_1$ Scintillator&1.032&0.507&0.523&58.50\\
A$_2$ Aerogel&0.22&5.00&1.100&66.30\\
AM Aerogel&0.10&9.00&0.900&66.30\\
Short Gas Cerenkov(CO$_2$)&0.1977E-02&100.00&0.197&62.40\\
S$_2$ Scintillator&1.032&0.52&0.536&58.50\\
Air (VDC1 to S$_2$ Scintillator)&0.121E-02&220.20&0.266&62.00\\
\hline \hline
$\lambda_I$&$\lambda_{avg}$&$\lambda_{act}$&X/$\lambda_{avg}$&X/$\lambda_{act}$ \\
(gm/cm$^2$)&(gm/cm$^2$)&(gm/cm$^2$)& &                                           \\
\hline \hline
50.80&47.05&46.7511&0.2557E-02&0.2573E-02\\
106.40&88.50&84.8795&0.5018E-03&0.5232E-03\\
106.40&88.50&84.8795&0.1006E-02&0.1049E-02\\
85.80&73.05&70.8246&0.4937E-03&0.5092E-03\\
124.90&102.40&97.4562&0.4433E-03&0.4658E-03\\
90.00&76.00&73.4211&0.1273E-02&0.1318E-02\\
85.70&74.10&72.2841&0.2251E-03&0.2307E-03\\
185.00&147.650&138.202&0.5228E-05&0.5586E-05\\
101.43&85.001&81.8256&0.2517E-03&0.2615E-03\\
81.90&70.20&68.25&0.7453E-02&0.7666E-02\\
96.90&81.60&78.7313&0.1348E-01&0.1397E-01\\
96.90&81.60&78.7313&0.1102E-01&0.1143E-01\\
89.70&76.05&73.60&0.2599E-02&0.2686E-02\\
81.90&70.20&68.25&0.7644E-02&0.7862E-02\\
90.00&76.00&73.4211&0.3505E-02&0.3628E-02\\
\hline \hline 
$\sum_{i=1}^n$(X/$\bar{\lambda}$)&  - & - &0.0525 & 0.0542 \\  
\hline 
Transmission  & - & - & 0.9488& 0.9472\\       
\hline \hline 
Absorption (\%)      & -    &   -    & 5.114  & 5.275  \\ 
\hline \hline
\end{tabular}
\caption[The absorbers used and their properties for the right arm spectrometer.]
{The absorbers used and their properties for the right arm spectrometer.}
\label{r_proton_absorp}
\end{center}
\end{table}
%%%%
\begin{table}[!htbp]
\begin{center}
\begin{tabular}{||c|c|c|c|c||}
\hline \hline
Target&Density&Thickness&X&$\lambda_T$\\
      &(gm/cm$^3$)&(cm)&(gm/cm$^2$)&(gm/cm$^2$)\\
\hline \hline
LH$_2$ Target&0.708E-01&1.94808&0.1379&43.30              \\
Al Target&2.70&0.147682E-01&0.3987E-01&70.60               \\   
Al Chamber&2.70&0.33E-01&0.891E-01&70.60                      \\
Kapton&1.42&0.254E-01&0.360E-01&60.30                        \\
Titanium&4.54&0.10E-01&0.454E-01&79.90                          \\
Air (Spectrometer exist to VDC1)&0.121E-02&80.00&0.968E-01&62.00 \\
Mylar (Wire Chamber)&1.39&0.12E-01&0.166E-01&62.50               \\
Wire VDC (effective)&19.30&0.40E-04&0.772E-03&110.30                \\ 
Ar/Ethan&0.107E-02&20.00&0.214E-01&68.572                           \\
S$_0$ Scintillator&1.032&1.00&1.032&58.50                             \\
S$_1$ Scintillator&1.032&0.507&0.523&58.50                          \\
A$_1$ Aerogel&0.60E-01&9.00&0.540&66.30                                  \\ 
Short Gas Cerenkov (CO$_2$)&0.1977E-02&100.00&0.197&62.40               \\
S$_2$ Scintillator&1.032&0.52&0.536&58.50                               \\
Air (VDC1 to S$_2$ Scintillator)&0.121E-02&220.20&0.266&62.00           \\
\hline \hline
$\lambda_I$&$\lambda_{avg}$&$\lambda_{act}$&X/$\lambda_{avg}$&X/$\lambda_{act}$ \\
(gm/cm$^2$)&(gm/cm$^2$)&(gm/cm$^2$)& &                                           \\
\hline \hline
50.80&47.05&46.7511&0.2931E-02&0.2950E-02                                 \\
106.40&88.50&84.8795&0.4505E-03&0.4697E-03                                 \\
106.40&88.50&84.8795&0.1006E-02&0.1049E-02                                  \\
85.80&73.05&70.8246&0.4937E-03&0.5092E-03                                    \\
124.90&102.40&97.4562&0.4433E-03&0.465E-03                                   \\
90.00&76.00&73.4211&0.1273E-02&0.1318E-02                                      \\
85.70&74.10&72.2841&0.2251E-03&0.2307E-03                                       \\
185.00&147.65&138.202&0.5228E-05&0.5586E-05                                     \\
101.43&85.001&81.8256&0.2517E-03&0.2615E-03                                      \\ 
81.90&70.20&68.25&0.1470E-01&0.1512E-01                                          \\
81.90&70.20&68.25&0.7453E-02&0.7666E-02                                          \\
96.90&81.60&78.7313&0.6617E-02&0.6858E-02                                         \\
89.70&76.05&73.60&0.2599E-02&0.2686E-02                                            \\
81.90&70.20&68.25&0.7644E-02&0.7862E-02                                            \\
90.00&76.00&73.4211&0.3505E-02&0.3628E-02                                           \\
\hline \hline 
$\sum_{i=1}^n$(X/$\bar{\lambda}$)&  - & - & 0.0496& 0.0510\\  
\hline 
Transmission  & - & - & 0.9516& 0.9502\\       
\hline \hline 
Absorption (\%)      & -    &   -    & 4.839& 4.980\\ 
\hline \hline
\end{tabular}
\caption[The absorbers used and their properties for the left arm spectrometer.]
{The absorbers used and their properties for the left arm spectrometer.}
\label{l_proton_absorp}
\end{center}
\end{table}

  

   


